Fully dynamic maximal matching in O(log n) update time

We present an algorithm for maintaining maximal matching in a graph under addition and deletion of edges. Our data structure is randomized that takes O(log n) expected amortized time for each edge update where n is the number of vertices in the graph. While there is a trivial O(n) algorithm for edge update, the previous best known result for this problem for a graph with n vertices and m edges is O({(n+ m)}^{0.7072})which is sub-linear only for a sparse graph. For the related problem of maximum matching, Onak and Rubinfield designed a randomized data structure that achieves O(log^2 n) amortized time for each update for maintaining a c-approximate maximum matching for some large constant c. In contrast, we can maintain a factor two approximate maximum matching in O(log n) expected time per update as a direct corollary of the maximal matching scheme. This in turn also implies a two approximate vertex cover maintenance scheme that takes O(log n) expected time per update.

==> conclusion-old.tex <==
\section{Conclusion}
We presented a fully dynamic randomized algorithm for maximal matching which 
achieves expected amortized $O(\log n)$ time per edge insertion or deletion. 
Maximal matching is also 2-approximation of maximum matching. 

\begin{comment}
We executed our algorithm on random graphs of various densities and found that
the matching maintained is very close to the maximum matching. But it is not 
hard to come up with an update sequence such that at the end of the sequence, 
the matching obtained is strictly half the size of maximum matching. 
We present one such example as follows (see Figure \ref{Figure8}). 
Let $G( V \cup U  , E)$ be a graph such that $V = \{v_1, v_2, \dots , v_n\}$ 
and $U = \{u_1, u_2, \dots, u_n\}$ for some even number $n$. Consider the 
following update sequence. In the first phase, add edges between every pair of
vertices present in $V$.
This results in a complete subgraph on vertices of $V$. 
The size of any maximal matching on a complete graph of size $n$ is $n/2$. 
After the first phase of updates ends, the size of matching obtained by our 
algorithm is $n/2$. In the second phase, add edge $(v_i,u_i)$ for all $i$. 
Note that the degree of each $u_i$ is one at the end of the updates. 
Let us now find the matching which our algorithm maintains.
Let $(v_i,v_j)$ be an edge in the matching after phase 1. Note that both 
these endpoints are at a level greater than -1. A vertex in $U$ is at level -1 
as it does not have any adjacent edges after phase 1. When an edge 
$(u_i,v_i)$ is added, since $v_i$ is at a higher level than $u_i$,
$v_i$ becomes the owner of this edge. The second invariant of $v_i$ is not
violated after this edge insertion and nothing happens at this update step 
and $u_i$ still remains at level -1. Using same reasoning, we can show that 
$u_j$ also remains at level -1 after the addition of edge $(v_j,u_j)$. 
So matching maintained by the algorithm remains unchanged. It is easy to 
observe that the maximum matching of the graph $G$ now has size $n$ which is 
twice the size of the matching maintained by our algorithm.
\begin{figure}[!t]
\centerline{\epsfysize=200pt \epsfbox{Figures/Clique.eps}}
\caption{An example where our algorithm gives a 2-approximation. The vertices on top 
are in $V$ and form a complete graph. The vertices at the bottom of the figure are 
in $U$.}
\label{Figure8}
\end{figure}
\end{comment} 

%{\color{red} 
Subsequent to the publication of the preliminary version of our 
article, there has been some interesting progress in the area of dynamic 
matching.
Neiman and Solomon \cite{NeimanS12} designed an algorithm that 
maintains a $3/2$-approximate matching 
in $O(\sqrt{m})$ time per update in general graphs. 
A similar result was also obtained concurrently and independently by 
Anand \cite{Anand-mtech-thesis}. These results were significantly improved
by Gupta and Peng \cite{GuptaP13}, where they designed an algorithm that 
maintains a $(1+\epsilon)$-approximate maximum matching in 
$O(\sqrt m \epsilon^{-2})$ update time for any $\epsilon>0$. 

Dynamic algorithms have also been designed for weighted matching.
Based on the algorithm in this paper,
Anand et al. \cite{AnandBGS12,AnandBGS-Arxiv12} designed a randomized 
algorithm that maintains a matching with a weight that is {\em expected} to be 
at least $1/4.9108\approx0.2036$ of the optimum. 
Later, Gupta and Peng \cite{GuptaP13} designed an algorithm that maintains a 
$(1+\epsilon)$-approximate weighted matching in 
$O(m \epsilon^{-O(1/\epsilon)}\log N)$ update time where the edges have 
weights in the range $[1,N]$.

One of the technical challenges in theoretical computer science is to prove 
lower bounds for algorithmic problems. Recently there has been some 
progress on proving conditional lower bounds for dynamic graph algorithms
\cite{Patrascu10,AbboudW14}. 
\begin{comment}
These lower bound results are conditioned
on some popular conjectures on the running time of some fundamental problems,
e.g., 3SUM, All-Pairs Shortest Paths, and Boolean Matrix Multiplication.
Abboud and Williams \cite{AbboudW14} showed that it might not be possible to 
achieve an approximation factor arbitrary close to 1 by any dynamic 
algorithm for matching that is based on augmenting paths. Notice that
if there is no augmenting path of length $\le 2k-3$, then the matching is
$k/(k-1)$-approximattion of the maximum matching. 
Abbound and Williams \cite{AbboudW14} showed that there is a constant 
$k\le 10$ such that if a dynamic algorithm maintains a matching such that
there is no augmenting path of length $\le 2k-3$,
then the update time taken by this algorithm must be $\Omega(m^{\epsilon})$ 
where $\epsilon > 1/3$ unless 3SUM has an $o(n^2)$ algorithm. 
%They also show similar lower bounds for maintaining 
%maximum cardinality bipartite matching and maximum weight bipartite matching.
%Note that these lower bounds are conditioned on some popular 
%conjecture, e.g, 3SUM conjecture. 
\end{comment}
In the light of the lower bound presented by Abboud and Williams 
\cite{AbboudW14} based on $\Omega(n^2)$ hardness of the 3SUM problem,
it would be an interesting and challenging problem to see 
if $c$-approximate maximum matching for $c<2$ can be maintained in $o(n)$ 
update time.




==> conclusion.tex <==
\section{Conclusion}
We presented a fully dynamic randomized algorithm for maximal matching which 
achieves expected amortized $O(\log n)$ time per edge insertion or deletion. 
Maximal matching is also 2-approximation of maximum matching. 
An interesting question is to explore how crucial randomization is for dynamic maximal matching.
Recently, Bhattacharya et al. \cite{DBLP:conf/stoc/BhattacharyaHN16} almost answered this question in affirmative by designing a determinstic algorithm that maintains $(2+\epsilon)$-approximate matching in amortized $O(poly (\log n, 1/\epsilon)$ update time. 
Another interesting question is to explore whether we can achieve $O(1)$ amortized update time. Very recently Shay \cite{DBLP:journals/corr/Solomon16} answered this question in affirmative as well by designing a randomized algorithm that takes $O(t + n \log n)$ update time with high probability to process any sequence of $t$ edge deletions. Though the basic building blocks of his algorithm are the same as ours, 
the two algorithms are inherently different and so are their analysis.

In our algorithm, a vertex may rise to a higher level and create a new epoch even when its matched
edge is intact. But Shay's algorithm takes a lazy approach to maintain the hierarchy of vertices
wherein a vertex is processed only when it becomes absolutely necessary. Another crucial difference is the following.
Our algorithm maintains a function $\phi_v(j)$ for each vertex $v$ and each level $j$.
This function is used to ensure an invariant that each vertex $v$ is at the highest possible level $\ell$ such that the edges incident from
lower levels is at least $4^{\ell}$. An important property guaranteed by this invariant is that the mate of a vertex while creating an epoch
is independent of the update sequence associated with the epoch. The analysis of our algorithm crucially exploits this property. 
However, the explicit maintenance of $\phi_v(j)$ imposes an overhead of $\Theta(\log n)$ in the update time. In order to achieve $O(1)$ update time, Shay \cite{DBLP:journals/corr/Solomon16} gets rid of the maintenance of $\phi_v(j)$ by taking a lazy approach and a couple of new ideas. As a result, unfortunately, the property of our algorithm no longer holds for the algorithm of Shay -  indeed there is dependence
between the update sequence associated with an epoch created by a vertex and the random mate picked by it. 
Shay makes use of a new concept called {\em uninterrupted duration} of an epoch that bypasses the
need of our property for the analysis. His analysis can be adapted to our algorithm as well. However, our analysis has its own merits
since it is based on an insightful property of our algorithm which we believe is of its own independent interest and importance.

Subsequent to the publication of the preliminary version of our 
article, there has been interesting progress in the area of dynamic 
matching with approximation less than 2 \cite{DBLP:conf/icalp/BernsteinS15, DBLP:conf/soda/BernsteinS16, NeimanS12, GuptaP13}, and
dynamic weighted matching \cite{AnandBGS12,AnandBGS-Arxiv12,GuptaP13}.

One of the technical challenges in theoretical computer science is to prove 
lower bounds for algorithmic problems. Recently there has been some 
progress on proving conditional lower bounds for dynamic graph algorithms
\cite{AbboudW14, DBLP:conf/stoc/HenzingerKNS15}. 
In the light of the lower bound presented by Abboud and Williams 
\cite{AbboudW14} based on $\Omega(n^2)$ hardness of the 3SUM problem,
it would be an interesting and challenging problem to see 
if $c$-approximate maximum matching for $c<2$ can be maintained in $o(n)$ 
update time.




==> few-random-bits.tex <==
\section{Reducing the number of random bits used by the algorithm}
At the start of each epoch, our algorithm selects a  
random number from $[1,...,M]$ . In case of our 2-\LL ~algorithm, we do it 
for \LL~ 1 only and $M \in [\sqrt{n},n]$; whereas in case of our final
algorithm, we do it for each \LL $\ge 0$, and $M \in [2^i, 2^{i+1}-1]$ for 
level $i$. Lemma \ref{lem:termination} (and Lemma \ref{lem:logntermination}) provide
a bound on the expected number of natural epochs terminated at 
\LL 1 (\LL~$i$) during $t$ updates at that level. Their proof required 
independence among the random numbers generated for various epochs, that is,
$O(\log n)$ truly random bits are used for each epoch. This implies that, in 
order to achieve expected amortized $O(\log n)$ update time, our algorithm
uses $O(\log n)$ random bits per edge update.
We shall now that our algorithm achieves the same asymptotic bound on the 
update time using much fewer random bits. In particular, if our algorithm uses 
only 4-wise independent random numbers, even then the expected number of 
natural epochs terminated during a sequence of $t$ updates at that 
level will be $\EX[X_t] = 16t/M + O(1)$.
We shall use the following Theorem, which can be viewed as an
extension of Chernoff bound for the case of sum of partially independent 
0-1 random variables.
\begin{theorem}{\cite{bernard,ssen}}
Let $x_1,x_2,\dots, x_n$ be $2k$-wise independent 0/1 random variables each equal to 1 with probability $p$.
There is an absolute constant $\beta$ such that for any constant $\alpha >0$,
\[\PP[ |X - np| \ge \alpha np] \le \big(\frac{\beta}{\alpha^2 np}\big)^k\]
where $X=x_1+x_2+\dots+x_n$.
\label{theorem61}
\end{theorem}

Let $Y_i$ be a $\log n$ bit random number generated by the algorithm for epoch $i$. Let 
these $Y_i$'s be 4-wise independent. Each $Y_i$ takes value from 
$[1 \dots M]$ with probability $1/M$. Let $Y_i^\tau$ be a random variable 
defined as follows:
\begin{equation}
Y_i^\tau = \left\{ 
   \begin{array}{ll} 
              1 &  \mbox{if~} Y_i \in [1, \dots, \tau] \\\\
              0 & \mbox{otherwise~}  
    \end{array}
  \right.
\end{equation}

Similar to Lemma~\ref{lemma34}, we can state that 
%
\begin{equation}
\PP[ Y_i^\tau = 1] \le \tau/M
\label{equation4}
\end{equation}
%
\begin{lemma}
For a given fixed $\tau\le M$, $Y_i^\tau$'s are 4-wise independent 0-1 random 
variables.
\label{lemma61}
\end{lemma}
\begin{proof}
Consider any 4-tuples $j_1,\ldots,j_4$. 
\begin{eqnarray*}
\PP[ Y_{j_1}^\tau=1 | Y_{j_2}=\omega_2, \ldots, Y_{j_4}=\omega_4]
& = & \PP[ Y_{j_1} \le \tau | Y_{j_2}=\omega_2, \ldots, Y_{j_4}=\omega_4]\\
& = & \PP[ Y_{j_1} \le \tau ] ~~~~~\mbox{\{since $Y_i$'s are 4-wise independent\}}\\
& = & \PP[Y_{j_1}^\tau=1]
\end{eqnarray*}
Hence $Y_i^\tau$'s are 4-wise independent.
\end{proof}

We now introduce the notion of good and bad epoch. We call an epoch to be a bad 
epoch if its duration is less than $\tau = M/4$, otherwise we call it a good 
epoch. It follows from Equation \ref{equation4} that an epoch is bad with 
probability at most $1/4$. Consider a sequence of $q$ epochs and let $Y$ be 
the random variable for the number of bad epochs among them.
Observe that the event ``$i$th epoch is bad'' is equivalent to
``$Y_i^\tau=1$''. It follows that $Y=\sum_i Y_i^\tau$. Hence, using linearity
of expectation, $\EX[Y]=q/4$. We shall now 
bound the probability for the event ``$Y\ge 3q/4$''.  Since $Y_i^\tau$'s
are 4-wise independent, we can apply Theorem \ref{theorem61} with $k=2$ to get
\begin{eqnarray*}
\PP[Y\ge 3q/4] & = & \PP[Y - q/4 \ge q/2]\\
               & \le & \left(  \frac{\beta}{q} \right)^2 
\end{eqnarray*}.

Let $X_t$ be the random variable for the number of natural epochs
that get terminated during $t$ updates. Fix $q_0=16t/M$. 
It follows from elementary probability theory  that
\begin{equation}
\EX[X_t] \le q_0 + \sum_{q>q_0} \PP[X_t \ge q]
\label{equation5}
\end{equation}

In order to show that $\EX[X_t] = O(t/M)$, it suffices to show 
$\sum_{q>q_0} \PP[X_t \ge q]$ is $O(1)$ in Equation \ref{equation5}. 
Let us investigate the event ``$X_t \ge q$'', that is,
at least $q$ epochs terminated during $t$ updates. It is easy to observe 
that there can be at most $4t/M$ good epochs out of $q$ epochs. In other
words, the event ``$X_t \ge q$'' implies that in a sequence of 
$q$ epochs, the number of bad epochs turned out to be at least $q-4t/M$
which is at least $3q/4$ since $q>16t/M$. Therefore, the event ``$X_t \ge q$''
implies the event ``$Y\ge 3q/4$'' whose probability we have bounded by
$\left(  \frac{\beta}{q} \right)^2$. 
Plugging the bound on $\PP[X_t\ge q]$ into Equation \ref{equation4}, we get

\[ \EX[X_t]=16t/M + \sum_{q>q_0} \frac{\beta^2}{q^2} ~ =~ 16t/M + O(1)\]
Hence, the expected number of epochs is $O(t/M)$ even when
the algorithm uses 4-wise independent random numbers. 
It is well known that, for any $\alpha > 0$, it takes $4 \alpha \log k$ truly random bits to generate a total
of $k^{\alpha}$ random numbers that will be 4-wise independent and consist of $\alpha \log k$ 
bits each. It implies that, for handling any sequence of $n^{\alpha}$ updates in the 
graph, our algorithm will require only $4 \alpha \log n$ truly random bits. 
So we can state the following theorem.
\begin{theorem}
Maximal matching of a graph can be maintained fully dynamically by a randomized
algorithm that achieves expected $O(t \log n)$ computation time to handle 
$t$ updates and the total number of random bits used by the algorithm
will be $O((t/n^{\Omega(1)}) \log n)$.
\label{theorem-fewer-random-bits}
\end{theorem}

\begin{remark}
Along similar lines, it can be shown that the computation time to handle 
$t$ updates by our algorithm will be $O(t \log n + n \log^2 n)$ with high 
probability if we use $O(\log n)$-wise independent random numbers. As a result,
the total number of random bits used by the algorithm will be $O((t/n^{\Omega(1)})\log^2 n)$. 
\end{remark}






==> intro.tex <==
\section{ Introduction }
Let $G=(V,E)$ be an undirected graph on $n=|V|$ vertices and $m=|E|$ edges.
A matching in $G$ is a set of edges $M\subseteq E$ such that no two 
edges in $M$ share any vertex. The study of matchings satisfying various 
properties has remained the focus of graph theory for decades \cite{LP86}. It is
due to the elegant structure of matching that it also appears in 
various combinatorial optimization problems \cite{EdmondsJohnson73,Lawler76}. 
A few well studied matching problems are maximum cardinality matching 
\cite{Edmonds65,HopcroftKarp73,MicaliVazirani80,MuchaS04}, maximum weight 
matching \cite{GabowTarjan91,HuangKavitha12}, minimum cost matching 
(chapter 7, \cite{KleinbergTardos05}), stable matching \cite{GaleShapley62}, 
popular matching \cite{AbrahamIKM07}. Among these problems, the maximum 
cardinality matching problem has been studied most extensively.
A matching $M$ is of maximum cardinality if 
the number of edges in $M$ is maximum. A maximum cardinality matching
(MCM)
is also referred to as a {\it maximum matching}. A matching is said to be a 
{\it maximal} 
matching if it cannot be strictly contained in any other matching. It is well 
known that a maximal matching guarantees a 2-approximation of the maximum 
matching. Though it is quite easy to compute a maximal matching in $O(m+n)$ 
time, designing an efficient algorithm for maximum matching has remained a 
very challenging problem for researchers \cite{Edmonds65,MicaliVazirani80}. 
The fastest algorithm, till date, for maximum matching runs in $O(m\sqrt{n})$ 
time and is due to Micali and Vazirani \cite{MicaliVazirani80}. In this 
paper, we address the problem of maintaining a maximal matching in a dynamic graph.

Most of the graph applications in real life deal with graphs that are not 
static, viz., the graph changes over time caused by deletion 
and insertion of edges. This has 
motivated researchers to design efficient algorithms for various graph problems
in dynamic environment. An algorithmic graph problem is modeled in
the dynamic environment as follows. There is an online 
sequence of insertion and deletion of edges and the goal is to update
the solution of the graph problem after each edge update. A trivial way to 
achieve this is to run the best static algorithm for this problem after each
edge update; clearly this approach is wasteful.  
The aim of a dynamic graph algorithm is to maintain some clever data structure 
for the underlying problem such that the time taken to   
update the solution is much smaller than that of the best static algorithm.
There exist many efficient dynamic algorithms for various
fundamental problems in graphs \cite{BaswanaKS12,HolmLT01,RodittyZwick08,RodittyZwick12,Thorup07}. The challenges involved in the design of an efficient 
dynamic algorithm can be exemplified by the classical problem of undirected 
connectivity. In the static setting, the standard 
solution is based on DFS or BFS, that take $O(m+n)$ space and time. However, it 
took many years of persistent research 
\cite{Fred83,EppsteinGIN97,HenzingerKing99,HolmLT01,KapronKM13} till a fully 
dynamic algorithm with polylogarithmic update time could be designed for this 
problem. Unlike connectivity, relatively less attention has been paid to the 
design of dynamic algorithms for matching till now.

Ivkovi\'c and Llyod \cite{IvkovicLlyod94} designed the first fully dynamic algorithm for 
maximal matching with $O((n+m)^{0.7072})$ update time. In contrast, there 
exists a much larger body of work for maximum matching.
Sankowski \cite{Sankowski07} designed an algorithm for maintaining maximum 
matching which processes each update in $O(n^{1.495})$ time.
Alberts and Henzinger \cite{AlbertHenzinger95} designed an expected $O(n)$ 
update time algorithm for maintaining maximum matching in a 
restricted update model where the edge being inserted (or deleted) is chosen
randomly from the edges absent (present) in the graph.
The goal of a $\polylog(n)$ update time dynamic maximum matching 
algorithm appears to be too ambitious. In particular, even achieving a 
$o(\sqrt{n})$ bound on the update time would imply an improvement of the 
longstanding $O(m\sqrt{n})$ bound of the best static algorithm for maximum 
matching \cite{MicaliVazirani80}. 
So approximation appears to be inevitable if we wish to achieve really fast 
update time for maintaining matching.
Recently, Onak and Rubinfeld \cite{OnakRubinfeld10} presented a randomized 
algorithm for maintaining a $c$-approximate (for some unspecified large constant $c$) 
matching in a dynamic graph that takes $O(\log^2 n)$ expected amortized time
for each edge update. This matching is not necessarily maximal, as a maximal 
matching would imply a factor two approximate maximum matching. 
In particular, they pose the following question -

``Our approximation factors are large constants. How small can they be made with
polylogarithmic update time ? 
Can they be made 2 ? Can the approximation constant be made smaller than two 
for maximum matching ?..''

We resolve one of their central questions by presenting 
a fully dynamic algorithm for maximal matching which achieves
$O(\log n)$ expected amortized time per edge insertion or deletion.
Our algorithm uses randomization very crucially in order to handle the updates 
efficiently. The matching maintained (or the random bits used) by the algorithm
at any time is not known to the adversary for him/her to choose the updates 
adaptively. This oblivious adversarial model is also used in randomized 
data structures like universal hashing \cite{CarterW77}.

Our algorithm also implies a similar result for maintaining a two 
approximate vertex cover. It is also used as a basis 
for maintaining approximate maximum weight matching in a dynamic 
graph \cite{AnandBGS12}.





\section{An overview}
\label{sec:prob}
Let $M$ denote a 
matching of the given graph at any moment. Every edge of $M$ is called 
a {\em matched} edge and an edge in $E\backslash M$ is called an 
{\em unmatched} edge. For an edge $(u,v)\in M$, we define $u$ to be 
the {\em mate} of $v$ and vice versa. For a vertex $x$, 
if there is an edge incident to it in the matching $M$, then $x$ is a 
{\em matched} vertex; otherwise it is {\em free} or {\em unmatched}.

In order to maintain a maximal matching, it suffices to ensure 
that there is no edge $(u,v)$ in the graph such that both $u$ and $v$ are 
free with respect to the matching $M$. From this observation,  
an obvious approach will be to maintain the information for each vertex 
whether it is matched or free at any stage. When an edge $(u,v)$ is inserted, 
add $(u,v)$ to the matching if $u$ and $v$ are free. For a case when an 
unmatched edge $(u,v)$ is deleted, no action is required. Otherwise, for both 
$u$ and $v$ we search their 
neighborhoods for any free vertex and update the matching accordingly.  
It follows that each update takes $O(1)$ computation time except when 
it involves deletion of a matched edge; in this case the computation time is of 
the order of the sum of the degrees of the two vertices. 
So this trivial algorithm is quite efficient for {\em small} degree vertices, 
but could be expensive for {\em large} degree vertices. 
An alternate approach to handling deletion of a matched edge is to use a
simple randomized technique - a vertex $u$ is matched with a randomly chosen 
neighbor $v$. Following the standard adversarial model, it can be observed 
that an expected $\deg(u)/2$ edges incident to $u$ will be deleted 
before deleting the matched edge $(u,v)$. 
So the expected amortized cost per edge deletion for $u$ is roughly 
$O\Big( \frac{\deg(u)+\deg(v)}{\deg(u)/2}\Big)$. If $\deg(v)<\deg(u)$, 
this cost is $O(1)$; but if $\deg(v)\gg \deg(u)$, 
then it can be as bad as the trivial 
algorithm. We combine the idea of choosing a random mate and 
the trivial algorithm suitably as follows. 
We first present a fully dynamic algorithm which achieves 
expected amortized $O(\sqrt{n})$ time per update.
We introduce a notion of 
{\em ownership} of edges in which we assign an edge to that endpoint which has 
{\em higher} degree. 
We maintain a partition of the set of vertices into two levels : 0 and 1. 
Level 0 consists of vertices which own  {\em fewer} edges than an 
appropriate threshold and we handle the 
updates in level 0 using the trivial algorithm. Level 1 consists of 
vertices (and their mates) which own {\em larger} number of edges and we use 
the idea of random mate to handle their updates. In particular, a vertex 
chooses a random mate from its set of owned edges which ensures that it selects 
a neighbor having a lower degree.
 

A careful analysis of the $O(\sqrt{n})$ update time algorithm 
suggests that a {\em finer} partition of vertices may
help in achieving a better update time. This leads to our final algorithm which 
achieves expected amortized $O(\log n)$ time per update. 
More specifically, our algorithm maintains an invariant that can be informally 
summarized as follows.

{\em Each vertex tries 
to rise to a level higher than its current level, if, upon reaching that level, 
there are sufficiently large number of edges incident on it from lower levels. 
Once a vertex reaches a new level, it selects a 
random edge from this set and makes it matched. }

Note that we say that {\it "a vertex rises"} to indicate that the vertex moves to a higher level
and {\it "a vertex falls"} to indicate that the vertex moves to a lower level.
A vertex may also fall to a lower level if the number of edges incident to it 
decreases. But a vertex only uses its neighborhood information to decide 
whether to move to higher or lower level. %We will see that 
Overall, the vertices use
their local information to reach a global equilibrium state in which 
after each update each vertex is at the {\em right} level having
no incentive to either move above or below its current level.
 
\subsection{Related Work}
Onak and Rubinfeld  \cite{OnakRubinfeld10} also pursue an approach which is based on the
use of randomization to handle updates efficiently. Their algorithm maintains 
a partition of vertices into a hierarchy of $O(\log n)$ levels that is 
along the lines of Parnas and Ron  \cite{ron}. However, the algorithm
follows a global approach in building level $i$ of this hierarchy as follows. 
For level $i$, the algorithm maintains a subgraph consisting of vertices 
$V_i$ and their neighbors such that a random subset of these edges forms a 
matching of size $|V_i|/a$ with high probability for some constant $a > 1$. 
If the matching at level $i$ falls below a predefined threshold, then 
a new matching is computed for the vertices at level $i$. The algorithm
always tries to ensure that the number of matched edges at level $i$ is 
always greater than $|V_i|/a$. As a consequence, a free vertex at level $i$ 
may not get processed if the matching size at level 
$i$ is above this threshold. This is the reason that the matching maintained
by their algorithm is not maximal. Moreover, the approximation factor $a$ is 
an outcome of some probabilistic calculations using Chernoff bounds
that is chosen to be {\em sufficiently} large. 
Therefore, it is unlikely that any simple variation of 
this global approach can lead to a maximal matching. 

Our algorithm also maintains a hierarchical partitioning of vertices, but it is 
quite different from the scheme of Onak and Rubinfeld  \cite{OnakRubinfeld10}. 
As described earlier, the algorithm in \cite{OnakRubinfeld10} may not process
a vertex at level $i$ if the matching at level $i$ is above a certain 
threshold. 
On the other hand, our algorithm processes a vertex at level $i$ as soon 
as it becomes {\em free}. Irrespective of the matching size at level $i$, 
the algorithm tries to find a matched edge for this {\em free} vertex. 
This is a {\em vertex centric} approach for maintaining matching which 
ensures that the matching is maximal.
Our algorithm achieves significantly better results 
than  \cite{OnakRubinfeld10}, i.e., a guaranteed factor 2 matching. 
%----------2016-edit-begin
%The use of randomization is limited to selecting a random neighbor of a vertex
%and the $O(\log n)$ expected update time can be obtained using only $O( \log n)$
%purely random bits.
%----------2016-edit-ends

\subsection{Organization of the paper}
For a gentle exposition of the ideas and techniques, we first 
describe a simple but less efficient fully dynamic algorithm for maximal 
matching in Section 4. We present our final fully dynamic algorithm which achieves expected amortized $O(\log n)$ time per update
in Section 5. In Section 6, we illustrate an example of a dynamic graph that establishes the tightness of the approximation factor guaranteed by our algorithm. In the following section, we describe notations and elementary results from the probability theory that we shall use. 
%This algorithm maintains a 2-level partition of the 
%vertices and achieves expected amortized $O(\sqrt{n})$ time per update. 
%In section 3, we present our final fully dynamic algorithm which has 
%$O(\log n)$ levels and achieves expected amortized $O(\log n)$ time per update 
%(Theorem \ref{theorem41}). 
%----------2016-edit-begins
%Though our algorithms use randomization very
%crucially to achieve efficiency, we show in Section 5 that the number of 
%random bits required by our algorithm is polylogarithmic.
%----------2016-edit-ends

%All logarithms in this paper are with base 2 unless mentioned otherwise. 
%During the analysis of algorithms, we shall use the terminology 
%{\it very high probability} for those events whose probability is
%$1-n^c$ for some positive constant $c$.%, i.e., inverse polynomial.



==> preliminaries-2.tex <==
\section{Preliminaries}

\begin{itemize}
\item

\item

\end{itemize}


\subsubsection*{Asymmetric random walk on a line}
Consider a particle performing a discrete random walk on a line. In each step, it moves one unit to the right
with probability $p$ or to the left with probability $q=1-p$. Each move is independent of the moves made in the past. 
The following lemma holds if $p>q$.
%
\begin{lemma}
Suppose the random walk starts at location $\ell$ units to the right of the origin. Then the probability that it ever reaches origin 
within $\le L$ steps is at most
\[ \frac{1-(p/q)^L}{1-(p/q)^{L+\ell}} < \left(\frac{q}{p}\right)^{\ell}  \]
\label{lemma:asymmetric-random-walk}
\end{lemma}
The proof of Lemma \ref{lemma:asymmetric-random-walk} is sketched in Appendix as well.

